Robust Evaluation of Diffusion-Based Adversarial Purification

We question the current evaluation practice on diffusion-based purification methods. Diffusion-based purification methods aim to remove adversarial effects from an input data point at test time. The approach gains increasing attention as an alternative to adversarial training due to the disentangling between training and testing. Well-known white-box attacks are often employed to measure the robustness of the purification. However, it is unknown whether these attacks are the most effective for the diffusion-based purification since the attacks are often tailored for adversarial training. We analyze the current practices and provide a new guideline for measuring the robustness of purification methods against adversarial attacks. Based on our analysis, we further propose a new purification strategy improving robustness compared to the current diffusion-based purification methods.

==> tables/diffpure_ablation.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{cccc}
    \hline
        \multirow{2}{*}{Defense} & \multirow{2}{*}{Attack Step Size} & \multicolumn{2}{c}{Accuracy (\%)} \\
        & & Standard & Robust \\ \hline
        \multirow{4}{*}{SDE} & Adjoint 0.001 & \multirow{4}{*}{89.18±2.72} & 76.21±2.72 \\
        & Backprop 0.005 & & 51.52±0.67 \\
        & Backprop 0.01 & & 53.83±1.19 \\
        & Backprop 0.025 & & 64.84±0.93 \\ \hline
        \multirow{3}{*}{ODE} & ODE adjoint 0.01 & \multirow{3}{*}{91.37±0.86} & 73.52±1.04 \\
        & Backprop 0.01 & & 41.37±1.72 \\
        & Backprop 0.025 & & 39.69±0.94 \\ \hline
    \end{tabular}
    \caption{$t^*=1$}
    \label{fig:diffpure_ablation}
\end{table}

==> tables/diffpure_autoattack.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{cccc}
    \hline
        \multirow{2}{*}{Threat Model} & \multirow{2}{*}{Defense} & \multirow{2}{*}{Attack} & Robust \\
        & & & Accuracy (\%) \\ \hline
        \multirow{4}{*}{$\ell_\infty(\epsilon=8/255)$} & \multirow{2}{*}{ADP~\citep{Yoon2021AdversarialPW}} & PGD+EOT & 37.27±1.22 \\
        & & AutoAttack & 59.53±0.87 \\
        & \multirow{2}{*}{DiffPure~\citep{Nie2022DiffusionMF}}  & PGD+EOT & 51.25±0.67 \\
        & & AutoAttack & 63.60±0.81 \\ \hline
        \multirow{4}{*}{$\ell_2(\epsilon=0.5)$} & \multirow{2}{*}{ADP~\citep{Yoon2021AdversarialPW}} & PGD+EOT & 74.26±0.98 \\
        & & AutoAttack & 79.57±0.38 \\
        & \multirow{2}{*}{DiffPure~\citep{Nie2022DiffusionMF}}  & PGD+EOT & 82.11±0.66 \\
        & & AutoAttack & 81.70±0.84 \\ \hline
    \end{tabular}
    }
    \caption{Robust accuracy of DiffPure~\citep{Nie2022DiffusionMF} and ADP~\citep{Yoon2021AdversarialPW} against PGD+EOT and AutoAttack on CIFAR-10. Random version of AutoAttack is used.}
    \label{table:diffpure_autoattack}
\end{table}





% \begin{table}[!t]
%     \centering
%     \begin{tabular}{cccc}
%     \hline
%         \multirow{2}{*}{Defense} & \multirow{2}{*}{Attack} & \multicolumn{2}{c}{Accuracy (\%)} \\
%         & & Standard & Robust \\ \hline
%         \multirow{3}{*}{SDE (0.001)}  & PGD+EOT & \multirow{3}{*}{89.78} & 53.83 \\
%         & AA (Rand) & & 61.52 \\
%         & AA (Standard) & & 80.47 \\ \hline
%         \multirow{3}{*}{ODE (0.01)}  & PGD+EOT & \multirow{3}{*}{91.37} & 41.37 \\
%         & AA (Rand) & & 53.91 \\
%         & AA (Standard) & & 72.46 \\ \hline
%     \end{tabular}
%     \caption{Robust accuracy of DiffPure~\citep{Nie2022DiffusionMF} against PGD+EOT, and two versions of AutoAttack (AA): the rand version and the standard version on CIFAR-10 with $\ell_\infty$-norm bounded perturbations of size $\epsilon = 8/255$. Backpropagation is used for generating adversarial samples. The number in parentheses is the step size of denoising process for defense. The maximum forward step $t^*$ is 0.1 and the step size of denoising process is 0.01 for both SDE and ODE.}
%     \label{table:diffpure_autoattack}
% \end{table}

==> tables/evaluation_prior_defense.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{cccrr}
    \hline
        \multirow{2}{*}{Defense} & \multirow{2}{*}{Type} & \multirow{2}{*}{Evaluation Method} & \multicolumn{2}{c}{Robust Accuracy (\%)} \\
         & & & reported & ours \\ \hline
        ADP~\citep{Yoon2021AdversarialPW} & DSM+LD & PGD+EOT (BPDA+EOT) & 68.98±0.90* & 37.27±1.22 \\
        DiffPure~\citep{Nie2022DiffusionMF} & Diffusion & PGD+EOT (AutoAttack) & 77.80±1.24* & 51.25±0.67 \\
        GDMP~\citep{Wang2022GuidedDM} & Diffusion & PGD+EOT (BPDA+EOT) & 76.72±0.59* & 30.82±1.33 \\ \hline
        SODEF~\citep{kang2021stable}** & ODE & AutoAttack (AutoAttack) & 57.76 (53.69) & 49.28 \\
        DISCO~\citep{ho2022disco} & Implicit function & AutoAttack (BPDA) & 47.18 & 0.00 \\ \hline
    \end{tabular}
    \caption{Results of our evaluation of the five adaptive test-time defenses. The robust accuracy of each defense is measured using the evaluation method (and the parenthesis used in the original paper) with $\ell_\infty$-norm bounded perturbations of size $\epsilon = 8/255$ on CIFAR-10. * This is evaluated with a classifier different from that used in the original paper. ** This method uses an adversarially trained classifier. The robust accuracy of the underlying static classifier is 53.69\% (which is denoted in parentheses).}
    \label{table:overal_evaluation}
\end{table*}
